Physics Potential of a Few Kiloton Scale Neutrino Detector at a Deep Underground Lab in Korea

The demand for underground labs for neutrino and rare event search experiments has been increasing over the last few decades. Yemilab, constructed in October 2022, is the first deep ($\sim$1~km) underground lab dedicated to science in Korea, where a large cylindrical cavern (D: 20~m, H: 20~m) was excavated in addition to the main caverns and halls. The large cavern could be utilized for a low background neutrino experiment by a liquid scintillator-based detector (LSC) where a 2.26 kiloton LS target would be filled. It's timely to have such a large but ultra-pure LS detector after the shutdown of the Borexino experiment so that solar neutrinos can be measured much more precisely. Interesting BSM physics searches can be also pursued with this detector when it's combined with an electron linac, a proton cyclotron (IsoDAR source), or a radioactive source. This article discusses the concept of a candidate detector and the physics potential of a large liquid scintillator detector.

==> Physics/Reactor.tex <==
\subsection{Reactor neutrinos}

About 400 reactor neutrinos per year per kiloton LS is expected assuming 100\% detection efficiency and neutrino oscillation from all reactors in Korea (see Fig.~\ref{figs/f:Yemi_geoNu}).
The closest Hanul reactor complex is at about 65~km away (see Fig.~\ref{figs/f:handuk_map}) and it dominantly contributes to the reactor neutrino flux.

